A Refreshed Similarity-based Upsampler for Direct High-Ratio Feature Upsampling

Feature upsampling is a fundamental and indispensable ingredient of almost all current network structures for dense prediction tasks. Recently, a popular similarity-based feature upsampling pipeline has been proposed, which utilizes a high-resolution feature as guidance to help upsample the low-resolution deep feature based on their local similarity. Albeit achieving promising performance, this pipeline has specific limitations: 1) HR query and LR key features are not well aligned; 2) the similarity between query-key features is computed based on the fixed inner product form; 3) neighbor selection is coarsely operated on LR features, resulting in mosaic artifacts. These shortcomings make the existing methods along this pipeline primarily applicable to hierarchical network architectures with iterative features as guidance and they are not readily extended to a broader range of structures, especially for a direct high-ratio upsampling. Against the issues, we meticulously optimize every methodological design. Specifically, we firstly propose an explicitly controllable query-key feature alignment from both semantic-aware and detail-aware perspectives, and then construct a parameterized paired central difference convolution block for flexibly calculating the similarity between the well-aligned query-key features. Besides, we develop a fine-grained neighbor selection strategy on HR features, which is simple yet effective for alleviating mosaic artifacts. Based on these careful designs, we systematically construct a refreshed similarity-based feature upsampling framework named ReSFU. Extensive experiments substantiate that our proposed ReSFU is finely applicable to various types of architectures in a direct high-ratio upsampling manner, and consistently achieves satisfactory performance on different dense prediction applications, showing superior generality and ease of deployment.

==> misc/fig12_tab3.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.49\linewidth}
        \centering
\includegraphics[width=0.99\linewidth]{figs/head_segformer.pdf}
  % \vspace{-0.2cm}
  \caption{For SegFormer with hierarchical upsampling, (a) previous baselines execute the iterative $\times 2$ upsampling with utilizing $C3$, $C2$, and $C1$ as the guidance feature, respectively; (b) Our ReSFU only adopts the guidance $C1$ for the direct upsampling with different ratios.}
  \label{fig:head_segformer}
    \end{minipage}
    % \hfill
    \begin{minipage}{0.49\linewidth}
    \footnotesize
    \caption{Evaluation on ADE20K with SegFormer-MiT-B1 and SegFormer-MiT-B5. The best and second-best results are highlighted in bold and underlined, respectively.} 
    \vspace{-0.2cm}
        \centering
\renewcommand{\arraystretch}{1.14}
\scalebox{0.84}{\setlength{\tabcolsep}{1.4mm}{
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
 \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c|}{ SegFormer-MiT-B1} & \multicolumn{4}{c}{SegFormer-MiT-B5}   \\
  & mIoU & mAcc  & bIoU & Params & mIoU & mAcc & bIoU & Params  \\ 
\midrule
 Bilinear   & 40.97 & 51.73 & 24.89 & 13.72M & 49.13 & 60.69 & 32.32 & 82.01M  \\
  Deconv   & 40.73 & 51.25 & 23.78 & 15.29M  & 49.76 & 61.39 & 32.95 & 83.52M \\
  PixelShuffle~\cite{shi2016real} & 39.69 & 50.11 & 23.55   & 15.30M   & 50.09 & 61.69 &  33.11 & 83.59M \\
     Stack-JBU \cite{fu2024featup}  & 41.71 & 52.01  & 25.80 & 13.95M  & 49.53 & 60.72 & 32.89 & 82.24M \\ 
CARAFE~\cite{wang2019carafe}   & 42.75 & 53.96 & 27.09 & 14.16M  & \underline{50.45}  & \textbf{62.29}  & 33.78 & 82.45M \\
  IndexNet \cite{lu2019indices}  & 41.79 & 52.40 & 25.45&  26.32M  & 49.73 & 61.32 & 33.21 & 94.61M \\
  FADE~\cite{lu2022fade}  & 43.09 & \underline{53.89} & \textbf{28.33}  & 14.00M   &  {50.43} & 61.99 & \textbf{34.51} & 82.29M \\
  SAPA~\cite{lu2022sapa}   & 42.74 & 53.39 & {27.61} & 13.82M   &  49.61 &  61.11 & 34.02 & 82.11M \\
  DySample~\cite{liu2023learning}   & \underline{43.48} & 53.82 & 27.38 & 13.72M  &50.14  & 61.51 & 33.93 & 82.01M \\
   ReSFU   &\textbf{43.84}  & \textbf{54.75} & \underline{28.06}  & 13.86M  & \textbf{50.89} & \underline{62.00} &  \underline{34.40} & 82.15M  \\ 
\bottomrule
\end{tabular}}}
    \end{minipage}
\end{figure*}


% \begin{figure}[t]
%   \centering
%   % \vspace{-0.2cm}
% \includegraphics[width=0.99\linewidth]{figs/head_segformer.pdf}
%   \vspace{-0.2cm}
%   \caption{For SegFormer with hierarchical upsampling, (a) previous baselines execute the iterative $\times 2$ upsampling with utilizing $C3$, $C2$, and $C1$ as the guidance feature, respectively; (b) Our ReSFU only adopts the guidance $C1$ for the direct upsampling with different ratios.}
%   \label{fig:head_segformer}
% \end{figure}


% \begin{table}[t] 
% \footnotesize
% \caption{Evaluation on ADE20K with SegFormer-MiT-B1 and SegFormer-MiT-B5. The best and second-best results are highlighted in bold and underlined, respectively.} 
% \vspace{-2mm}
% \label{tab:segformer}
% \centering
% \renewcommand{\arraystretch}{1.14}
% \scalebox{0.84}{\setlength{\tabcolsep}{1.4mm}{
% \begin{tabular}{@{}l|cccc|cccc@{}}
% \toprule
%  \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c|}{ SegFormer-MiT-B1} & \multicolumn{4}{c}{SegFormer-MiT-B5}   \\
%   & mIoU & mAcc  & bIoU & Params & mIoU & mAcc & bIoU & Params  \\ 
% \midrule
%  Bilinear   & 40.97 & 51.73 & 24.89 & 13.72M & 49.13 & 60.69 & 32.32 & 82.01M  \\
%   Deconv   & 40.73 & 51.25 & 23.78 & 15.29M  & 49.76 & 61.39 & 32.95 & 83.52M \\
%   PixelShuffle~\cite{shi2016real} & 39.69 & 50.11 & 23.55   & 15.30M   & 50.09 & 61.69 &  33.11 & 83.59M \\
%      Stack-JBU \cite{fu2024featup}  & 41.71 & 52.01  & 25.80 & 13.95M  & 49.53 & 60.72 & 32.89 & 82.24M \\ 
% CARAFE~\cite{wang2019carafe}   & 42.75 & 53.96 & 27.09 & 14.16M  & \underline{50.45}  & \textbf{62.29}  & 33.78 & 82.45M \\
%   IndexNet \cite{lu2019indices}  & 41.79 & 52.40 & 25.45&  26.32M  & 49.73 & 61.32 & 33.21 & 94.61M \\
%   FADE~\cite{lu2022fade}  & 43.09 & \underline{53.89} & \textbf{28.33}  & 14.00M   &  {50.43} & 61.99 & \textbf{34.51} & 82.29M \\
%   SAPA~\cite{lu2022sapa}   & 42.74 & 53.39 & {27.61} & 13.82M   &  49.61 &  61.11 & 34.02 & 82.11M \\
%   DySample~\cite{liu2023learning}   & \underline{43.48} & 53.82 & 27.38 & 13.72M  &50.14  & 61.51 & 33.93 & 82.01M \\
%    ReSFU   &\textbf{43.84}  & \textbf{54.75} & \underline{28.06}  & 13.86M  & \textbf{50.89} & \underline{62.00} &  \underline{34.40} & 82.15M  \\ 
% \bottomrule
% \end{tabular}}}
% \vspace{-3mm}
% \end{table}


==> misc/fig_head.tex <==
\begin{figure*}[t]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/head5.pdf}
  % \vspace{-0.25cm}
  \caption{Incorporation of the proposed ReSFU into different network backbones. More details are provided in \textit{SM}.}
  \label{fig:head}
  % \vspace{-0.2cm}
\end{figure*}



==> misc/fig_head_fpn.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/head_fpn.pdf}
  \vspace{-0.2cm}
  % \caption{Illustration of the architecture of the FPN neck. (a) For previous methods requiring guidance information, they sequentially use $C3$, $C2$, and $C1$ as guidance features; (b) ReSFU use (rescaled) $C1$ as guidance feature in all involved upsampling modules. }
  \caption{For MaskFormer with the FPN neck, (a) previous methods sequentially take $C3$, $C2$, and $C1$ as guidance to execute the $\times 2$ upsampling; (b) Our ReSFU directly utilizes $C1$ to guide the upsampling for different levels of features.}
  \label{fig:head_fpn}
  \vspace{-2mm}
\end{figure}



==> misc/fig_head_psp.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/head_psp.jpg}
  \vspace{-0.2cm}
  % \caption{The incorporation manner of feature upsampling methods in PSPNet. The initial feature represents the intermediate feature obtained after applying the stem convolutions to the input image. (a) For compared upsampling methods adopt two $\times 2$ upsampling processes by default for better stability; (b) ReSFU directly performs a $\times 4$ upsampling process under the guidance of the initial feature.}
  \caption{For the CNN-based PSPNet with non-hierarchical upsampling, (a) previous baselines adopt a two-step upsampling by default; (b) Our ReSFU performs a one-step $\times 4$ upsampling. The guidance feature is from the involved stem ConvBlock layer in the ResNet backbone.}
  \label{fig:head_psp}
  \vspace{-2mm}
\end{figure}



==> misc/fig_head_segformer.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/head_segformer.pdf}
  \vspace{-0.2cm}
  \caption{For SegFormer with hierarchical upsampling, (a) previous baselines execute the iterative $\times 2$ upsampling with utilizing $C3$, $C2$, and $C1$ as the guidance feature, respectively; (b) Our ReSFU only adopts the guidance $C1$ for the direct upsampling with different ratios.}
  \label{fig:head_segformer}
  \vspace{-2mm}
\end{figure}



==> misc/fig_head_segmenter.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/head_segmenter.jpg}
  \vspace{-0.2cm}
  % \caption{The incorporation manner of feature upsampling methods in Segmenter. The guidance feature is generated by the convolution results of the input image. (a) The compared methods adopt two $\times 2$ upsampling processes by default for better stability; (b) ReSFU directly performs a $\times 4$ upsampling process.} 
\caption{For the Transformer-based Segmenter with non-hierarchical upsampling, (a) previous methods adopt two $\times 2$ upsampling processes; (b) Our ReSFU directly performs a $\times 4$ upsampling. The guidance HR feature is obtained by applying an additional ConvBlock to the input image.}
  \label{fig:head_segmenter}
  % \vspace{-3mm}
\end{figure}



==> misc/fig_vis_ins_pano.tex <==
\begin{figure*}[!t]
  \centering
  % \vspace{-0.7cm}
  % \vspace{-2mm}
\includegraphics[width=0.99\linewidth]{figs/vis_ins_pano.pdf}
  % \vspace{-0.4cm}
  \caption{Visualization results of different methods for instance segmentation (upper row) and panoptic segmentation (lower row).}
  \label{fig:vis_ins}
  % \vspace{-0.4cm}
\end{figure*}


==> misc/fig_vis_semantic.tex <==
\begin{figure*}[!h]
  \centering
  % \vspace{-0.2cm}
\includegraphics[width=0.99\linewidth]{figs/vis_semantic.pdf}
  % \vspace{-0.4cm}
  \caption{Visual comparison of upsampled features and prediction masks for semantic segmentation. \textit{Best viewed with zoom-in.}}
  \label{fig:vis_seg}
  % \vspace{-0.3cm}
\end{figure*}



==> misc/tab_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \small
% \vspace{-0.3cm}
% \caption{Ablation study on our specific designs, including .... \vspace{-3mm}}
% \label{tab:ablation}
% \centering
% \renewcommand{\arraystretch}{0.99}
% \setlength{\tabcolsep}{1.9mm}{
% \begin{tabular}{@{}c|ccccc|cc@{}} 
% \toprule 
% Variants & NS & GF & $\bm{s}_s$ & $\bm{s}_d$  & PCD & mIoU & bIoU \\ \hline
% (a) & \grey{\xmark}  &   \hazel{\cmark} & \hazel{\cmark} &  \hazel{\cmark} & \hazel{\cmark} & 46.69 &     \\
% (b)& \hazel{\cmark}  & \grey{\xmark}  &  \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} & 46.59 &     \\
% (c)& \hazel{\cmark} & - & \grey{\xmark}  & \hazel{\cmark} & \hazel{\cmark} & 46.46 &  \\
% (d)& \hazel{\cmark} &   \hazel{\cmark}  &  \hazel{\cmark}& \grey{\xmark} & \hazel{\cmark} & 46.92 &   \\ 
% (e)& \hazel{\cmark} & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} &  \grey{\xmark} & 46.26 &   \\ 
% (f)& \hazel{\cmark} & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} &  T & 46.43 &   \\ \hline
% (g) & \hazel{\cmark} & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} & \hazel{\cmark}  & 47.09 &   \\ \bottomrule
% \end{tabular} } \vspace{-6mm}
% \end{table}


% \begin{table}[]
% \footnotesize
% \vspace{-0.3cm}
% \caption{Ablation study on our specific designs, including .... \vspace{-3mm}}
% \label{tab:ablation}
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{1.1mm}{
% \begin{tabular}{@{}c|ccccc|ccccc@{}} 
% \toprule 
%  & $\bm{s}_s$ & NS & PCD & GF  & $\bm{s}_d$   & mIoU & mAcc & bIoU &FLOPs & Params \\ \hline
% (a) & \hazel{\cmark}  &   \grey{\xmark} & \grey{\xmark} &  \grey{\xmark} & \grey{\xmark} & 45.70  &  & & & \\
% (b)& \hazel{\cmark}  & \hazel{\cmark}  &  \grey{\xmark}  & \grey{\xmark}  & \grey{\xmark} & 45.80 &   & & &   \\
% (c)& \hazel{\cmark} & \hazel{\cmark} & \hazel{\cmark}  & \grey{\xmark} & \grey{\xmark} & 46.46 &  & & & \\
% (d)& \hazel{\cmark} &   \hazel{\cmark}  &  \hazel{\cmark}& \hazel{\cmark} & \grey{\xmark} & 46.92 &  & & &  \\ 
% (e)& \grey{\xmark} &   \hazel{\cmark}  &  \hazel{\cmark}& \grey{\xmark} & \hazel{\cmark} & 46.55 &  & & &  \\ \hline
% (f) & \hazel{\cmark} & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} & \hazel{\cmark}  & 47.09 &   & & & \\ \bottomrule
% \end{tabular} } \vspace{-6mm}
% \end{table}

\begin{table}[!t]
\footnotesize
% \vspace{-0.3cm}
\caption{Ablation study based on Segmenter-S. Variant (a) is the bilinear upsampler. In variants (b) and (c), $\bm{s}_{s}$ is computed based on the original $\bm{q}$ and $\tilde{\bm{k}}$ in Fig.~\ref{fig:main} (b) without GF optimization. `\grey{\xmark}' for PCDC means using inner product in Eq.~\eqref{eqn:sapa} for similarity calculation. `-' for PCDC means replacing the PCDC in PCDC-Block with the plain dilated convolution by concatenating $\bar{\bm{q}}$ and $\bar{\bm{k}}$ in Fig.~\ref{fig:pcd}. {FLOPs are tested with the image size of 512 $\times$ 512.} }\vspace{-3mm}
\label{tab:ablation}
\centering
\renewcommand{\arraystretch}{1.14}
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{@{}c|ccccc|ccccc@{}} 
\toprule 
Variant & $\bm{s}_s$  & PCDC & GF  & $\bm{s}_d$  & FNS & mIoU & mAcc & bIoU &FLOPs & Params \\ \hline
 (a)& \grey{\xmark}  &  \grey{\xmark}  & \grey{\xmark}  & \grey{\xmark} & \grey{\xmark} & 45.75 & 56.88  & 27.82 & 32.77G & 22.04M \\
(b)& \hazel{\cmark}  &  \grey{\xmark}  & \grey{\xmark}  & \grey{\xmark}& \hazel{\cmark} & 45.80 & 56.95  & 28.61 & 33.21G & 22.08M   \\
(c)& \hazel{\cmark} & \hazel{\cmark}  & \grey{\xmark} & \grey{\xmark}& \hazel{\cmark} &  &  &  & 33.48G & 22.09M \\
(d)& \hazel{\cmark}  &  \hazel{\cmark}& \hazel{\cmark} & \grey{\xmark}& \hazel{\cmark} &  &  &  & 33.49G & 22.09M  \\ 
(e)& \grey{\xmark}   &  \hazel{\cmark}& \grey{\xmark} & \hazel{\cmark}& \hazel{\cmark} &   &  &  & 33.47G & 22.08M \\ 
(f)& \hazel{\cmark}   &  -& \hazel{\cmark} & \hazel{\cmark}& \hazel{\cmark} &  &  &  & 34.15G & 22.12M \\ 
(g) & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} & \hazel{\cmark}& \grey{\xmark}  &  &  &  &  33.88G & 22.11M  \\ \hline
(h) & \hazel{\cmark}  & \hazel{\cmark}  & \hazel{\cmark} & \hazel{\cmark}& \hazel{\cmark}  & 46.97 & 57.91 & 29.96 & 33.88G & 22.11M \\ \bottomrule
\end{tabular} } %\vspace{-4mm}
\end{table}



==> misc/table_instance_old.tex <==
% \begin{table}[t] 
% \footnotesize
% % \vspace{-0.2cm}
% \caption{Instance segmentation and panoptic segmentation.}\vspace{-3mm}
% \label{tab:instance}
% \centering
% \renewcommand{\arraystretch}{1.05}
% \setlength{\tabcolsep}{0.5mm}{
% \begin{tabular}{@{}l|cccccc|ccccc@{}}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{6}{c|}{Instance Segmentation} & \multicolumn{5}{c}{Panoptic Segmentation} \\
%  & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ & PQ & PQ$^{th}$ & PQ$^{st}$ & SQ & RQ \\  \midrule
% Nearest & 34.7 & 55.8 & 37.2 & 16.1 & 37.3 & 50.8 & 40.2 & 47.8 & 28.9 & 77.8 & 49.3 \\
% Deconv & 34.5  & 55.5  & 36.8  & 16.4  & 37.0  & 49.5  & 39.6  & 47.0  & 28.4  & 77.1  & 48.5 \\
% PixelShuffle~\cite{shi2016real} & 34.8  & 56.0  & 37.3  & 16.3  & 37.5  & 50.4  & 40.0  & 47.4  & 28.8  & 77.1  & 49.1 \\
% CARAFE~\cite{wang2019carafe} &  35.4 &  56.7 & 37.6 & \underline{16.9}  & 38.1  & 51.3  & 40.8  & 47.7  & 30.4  & 78.2  & 50.0 \\
% IndexNet~\cite{lu2019indices} & 34.7 & 55.9  & 37.1 & 16.0 & 37.0  & 51.1 & 40.2 &  47.6 & 28.9 &  77.1 & 49.3 \\
% A2U~\cite{dai2021learning} & 34.6 & 56.0 & 36.8  &  16.1 &  37.4 & 50.3  &  40.1 & 47.6  & 28.7  &  77.3 & 48.0 \\
% FADE~\cite{lu2022fade} & 35.1 & 56.7 &  37.2 &  16.7 &  37.5 & 51.4  &  40.9 &  48.0 & 30.3  & 78.1  & 50.1 \\
% SAPA-B~\cite{lu2022sapa} & 35.1 & 56.5  & 37.4  & 16.7  & 37.6  & 50.6  & 40.6  & 47.7  & 29.8  & 78.0  & 49.6 \\
% % DySample & 35.4  & 56.9 & 37.8 & 17.1 & 37.7  & 51.1  &  41.4 &  \textbf{48.5} &  30.7 & \textbf{78.6}  & \textbf{50.7} \\
% % DySample-S+ & 35.5 & 56.8 & 37.8  & 17.0  & 37.9  & 51.9  & 41.1  & 48.1  & 30.5  &  78.2 & 50.2 \\
% DySample+~\cite{liu2023learning} & \underline{35.7} & \underline{57.3}  &  \underline{38.2} &  \textbf{17.3} & \underline{38.2}  & \underline{51.8}  & \textbf{41.5}  & \textbf{48.5}  & \underline{30.8}  & \underline{78.3}  & \textbf{50.7} \\
% % Ours & 35.7  & 57.0  & 37.9  & 17.0  & 38.3  & 52.1  &  41.3 & 48.2  & 31.0  & 78.4  & 50.5 \\
% Ours &  \textbf{36.1} & \textbf{57.4} &  \textbf{38.4} & 16.8 & \textbf{38.8}  & \textbf{52.5}  & \textbf{41.5}  & \underline{48.4}   & \textbf{31.1}  & \textbf{78.4}  & \textbf{50.7} \\
% \bottomrule
% \end{tabular}}
% % \vspace{-1mm}
% \end{table}

\begin{table*}[t] 
% \footnotesize
\small
% \vspace{-0.2cm}
\caption{Performance evaluation on more tasks, including instance segmentation and panoptic segmentation.}%\vspace{-3mm}
\label{tab:instance}
\centering
\renewcommand{\arraystretch}{1.14}
\setlength{\tabcolsep}{1.8mm}{
\begin{tabular}{@{}l|cccccc|ccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{6}{c|}{Instance Segmentation} & \multicolumn{5}{c}{Panoptic Segmentation} \\
 & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ & PQ & PQ$^{th}$ & PQ$^{st}$ & SQ & RQ \\  \midrule
Nearest & 34.7 & 55.8 & 37.2 & 16.1 & 37.3 & 50.8 & 40.2 & 47.8 & 28.9 & 77.8 & 49.3 \\
Bilinear  & 34.4 & 55.4 & 36.7 & 15.6 & 36.9 & 51.2 & 40.1 & 47.5 & 28.9 & 77.8 & 49.1 \\
Deconv & 34.5  & 55.5  & 36.8  & 16.4  & 37.0  & 49.5  & 39.6  & 47.0  & 28.4  & 77.1  & 48.5 \\
PixelShuffle~\cite{shi2016real} & 34.8  & 56.0  & 37.3  & 16.3  & 37.5  & 50.4  & 40.0  & 47.4  & 28.8  & 77.1  & 49.1 \\
CARAFE~\cite{wang2019carafe} &  35.4 &  56.7 & 37.6 & \underline{16.9}  & 38.1  & 51.3  & 40.8  & 47.7  & 30.4  & 78.2  & 50.0 \\
IndexNet \cite{lu2019indices} & 34.7 & 55.9  & 37.1 & 16.0 & 37.0  & 51.1 & 40.2 &  47.6 & 28.9 &  77.1 & 49.3 \\
A2U \cite{dai2021learning} & 34.6 & 56.0 & 36.8  &  16.1 &  37.4 & 50.3  &  40.1 & 47.6  & 28.7  &  77.3 & 48.0 \\
FADE \cite{lu2022fade} & 35.1 & 56.7 &  37.2 &  16.7 &  37.5 & 51.4  &  \underline{40.9} &  48.0 & 30.3  & 78.1  & \underline{50.1} \\
SAPA-B \cite{lu2022sapa} & 35.1 & 56.5  & 37.4  & 16.7  & 37.6  & 50.6  & 40.6  & 47.7  & 29.8  & 78.0  & 49.6 \\
DySample+ \cite{liu2023learning} & \underline{35.7} & \underline{57.3}  &  \underline{38.2} &  \textbf{17.3} & \underline{38.2}  & \underline{51.8}  & \textbf{41.5}  & \textbf{48.5}  & \underline{30.8}  & \underline{78.3}  & \textbf{50.7} \\
Stack-JBU \cite{fu2024featup} & NA & NA  & NA & NA  & NA & NA  & 40.4  & 47.7  & 29.3  & 77.8  & 49.4 \\
ReSFU &  \textbf{36.1} & \textbf{57.4} &  \textbf{38.4} & 16.8 & \textbf{38.8}  & \textbf{52.5}  & \textbf{41.5}  & \underline{48.4}   & \textbf{31.1}  & \textbf{78.4}  & \textbf{50.7} \\
\bottomrule
\end{tabular}}
% \vspace{-5mm}
\end{table*}


==> misc/table_semantic.tex <==


\begin{table*}[t] 
\footnotesize
% \vspace{-0.2cm}
\caption{Evaluation on semantic segmentation, with the best and second-best results highlighted in bold and underlined, respectively.} 
\label{tab:semantic}
\centering
\renewcommand{\arraystretch}{1.14}
\setlength{\tabcolsep}{1.75mm}{
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{Method}} & \multicolumn{3}{c|}{ PSPNet-R50 \cite{zhao2017pyramid}} & \multicolumn{3}{c|}{Segmenter-S \cite{strudel2021segmenter}} & \multicolumn{3}{c|}{SegFormer-B1 \cite{xie2021segformer}} & \multicolumn{3}{c|}{SegNeXt-B \cite{guo2022segnext}}  & \multicolumn{3}{c}{UNet-S5-D16 \cite{ronneberger2015u}}    \\
 & \multicolumn{3}{c|}{ADE20K \cite{zhou2017scene}} & \multicolumn{3}{c|}{ADE20K \cite{zhou2017scene}} & \multicolumn{3}{c|}{ADE20K \cite{zhou2017scene}} & \multicolumn{3}{c|}{ADE20K \cite{zhou2017scene}}  & \multicolumn{3}{c}{Cityscapes \cite{cordts2016cityscapes}}    \\
 & mIoU & mAcc  & bIoU & mIoU & mAcc & bIoU   & mIoU & mAcc   & bIoU & mIoU & mAcc  & bIoU & mIoU & mAcc  & bIoU \\ 
\midrule
Bilinear  & 41.13  & 51.41  & 26.01 & 45.75  & 56.88 & 27.82 &  40.97 & 51.73 & 24.89  & 47.78  & 58.43  & 31.89 & 69.10  & 76.76 & 53.12 \\
Deconv  &  39.11 & 48.79 & 24.09 &  40.93 & 51.62 & 23.77 & 40.73 & 51.25 & 23.78  & 46.94 & 58.34 & 30.69 & 68.37  & 76.04 & 54.08 \\
PixelShuffle~\cite{shi2016real}  & 38.31  & 47.78 & 23.77  &  41.24 & 52.37 & 23.87 & 39.69 & 50.11 & 23.55 & 47.66  & 59.19 & 31.21 & 67.54  & 74.67  & 53.61 \\
CARAFE~\cite{wang2019carafe} &  \underline{42.08} & \underline{52.47} & 26.75  & \underline{46.22}  & \underline{57.59} & \underline{29.10} & 42.75 & 53.96 & 27.09 & 48.37  & 59.50 & 32.46 &  71.01 &  78.14 & 56.29 \\
FADE~\cite{lu2022fade}  & 41.97  & 52.18 & 26.87  & 45.52  & 56.81 & 28.13 & 43.09 & \underline{53.89} & \textbf{28.33} & 48.36  & 59.75 & \underline{32.51} & 70.70  & 78.06 & 56.00 \\
SAPA-B~\cite{lu2022sapa}  & 41.60  & 52.01 & \underline{26.94}  &  45.89 & 57.01 & 28.78 & 42.74 & 53.39 & \underline{27.61} &  47.73 & 58.99 & 32.08 & 73.42  & 80.47  & 58.19 \\
DySample-S+~\cite{liu2023learning}  & 41.39  & 51.30 & 26.27 & 45.09  &  55.98 & 27.73 & \underline{43.48} & 53.82 & 27.38  & \underline{48.74}  & \textbf{60.77} & 32.09 & \underline{74.19}  & \underline{81.11}  & \underline{58.56} \\
ReSFU  & \textbf{42.52}  & \textbf{53.04} & \textbf{27.94}   &  \textbf{47.15} & \textbf{58.35} & \textbf{30.22} & \textbf{43.80} & \textbf{54.68} & 27.48  &  \textbf{49.11} & \underline{60.62} & \textbf{32.80} & \textbf{74.91}  &  \textbf{81.87} & \textbf{58.82} \\
\bottomrule
\end{tabular}}
% \vspace{-1mm}
\end{table*}


==> misc/table_synapse_old.tex <==


\begin{table*}[t] 
% \footnotesize
\small
% \vspace{-0.2cm}
\caption{Evaluation on semantic segmentation, with the best and second-best results highlighted in bold and underlined, respectively.} 
\label{tab:synapse}
\centering
\renewcommand{\arraystretch}{1.14}
\setlength{\tabcolsep}{1.75mm}{
\begin{tabular}{@{}l|cccccccc|c@{}}
\toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{ PSPNet-R50} & \multicolumn{3}{c}{PSPNet-R101}   \\
\multicolumn{1}{c|}{Method} & Aorta & Gallbladder & Kidney (L) &  Kidney (R) &  Liver & Pancreas & Spleen & Stomach & Average \\
\midrule
Bilinear  & \underline{87.23} & 63.13 & \underline{81.87} & \underline{77.02} & 94.08 & 55.86 & 85.08 & 75.62 & 77.48 \\
% Deconv  & & & & & & & &  &    \\
% PixelShuffle~\cite{shi2016real}  & & & & & & & &  &    \\
CARAFE~\cite{wang2019carafe} & 86.59 & 59.23 & 81.07 & 76.15  & 93.47 & 51.55 & 83.35 & 75.67 & 75.88  \\
FADE~\cite{lu2022fade} & 86.51 & 63.20 & \textbf{82.51} & \textbf{78.03} & 93.91 & 54.74 & \underline{85.67} & \textbf{78.31} & \underline{77.86} \\
SAPA-B~\cite{lu2022sapa}  & 85.19 & 59.15 & 74.51 & 75.09 & 92.38 & 50.39 & 82.16 & 66.08 & 73.12 \\
DySample-S+~\cite{liu2023learning} & 87.00 & \underline{66.89} & 80.76 & 75.05 & \textbf{94.34} & \underline{56.87} & 84.44 & 76.00 & 77.67   \\
Stack-JBU \cite{fu2024featup} & 86.39 & 61.63 & 77.56 & 75.24 & 93.33 & 54.31 & 84.59 & 75.78  & 76.10  \\
ReSFU  & \textbf{87.49} & \textbf{67.17} & 81.59 & 76.00 & \underline{94.30} & \textbf{59.77} & \textbf{86.50} & \underline{76.97} & \textbf{78.72} \\
\bottomrule
\end{tabular}}
% \vspace{-1mm}
\end{table*}

